GeoDTR+: Toward generic cross-view geolocalization via geometric disentanglement

Cross-View Geo-Localization (CVGL) estimates the location of a ground image by matching it to a geo-tagged aerial image in a database. Recent works achieve outstanding progress on CVGL benchmarks. However, existing methods still suffer from poor performance in cross-area evaluation, in which the training and testing data are captured from completely distinct areas. We attribute this deficiency to the lack of ability to extract the geometric layout of visual features and models' overfitting to low-level details. Our preliminary work introduced a Geometric Layout Extractor (GLE) to capture the geometric layout from input features. However, the previous GLE does not fully exploit information in the input feature. In this work, we propose GeoDTR+ with an enhanced GLE module that better models the correlations among visual features. To fully explore the LS techniques from our preliminary work, we further propose Contrastive Hard Samples Generation (CHSG) to facilitate model training. Extensive experiments show that GeoDTR+ achieves state-of-the-art (SOTA) results in cross-area evaluation on CVUSA, CVACT, and VIGOR by a large margin ($16.44\%$, $22.71\%$, and $13.66\%$ without polar transformation) while keeping the same-area performance comparable to existing SOTA. Moreover, we provide detailed analyses of GeoDTR+. Our code will be available at https://gitlab.com/vail-uvm/geodtr plus.

==> text/response.tex <==
\textbf{\Large Summary of Changes} \\

We are deeply thankful to the reviewers for their perceptive and helpful feedback on our paper, ``GeoDTR+: Toward Generic Cross-View Geolocalization via Geometric Disentanglemen''. We value the time they invested and the thoughtful suggestions they provided to enhance the quality and clarity of our work.
We have revised the text, table, and figures in the manuscript to address the possible confusions identified by the reviewer. We also carried out extra experiments suggested by the reviewer to further clarify our contribution and improve the comprehensibility of this work. Below, we provide a point-to-point response to the questions and concerns of the reviewer.\\


\q{The difference between the two pathways.}

\answer{The two-pathway design is central for our \ourmodel{}, where the Backbone Feature Pathway \textbf{replicates} the raw backbone features from the backbone network and the Geometric Layout Pathway is \textbf{solely} devoted to \textbf{explicitly model} the layout information. The outputs from the two pathways fuse according to~\Cref{eq:main} to produce the final latent representations. We agree with the reviewer that \Cref{eq:main} is symmetric in its appearance. However, elements of descriptors $\mathbf{q}$ take values in $[0,1]$ while there is no such constraint on the backbone features. In this sense, the two pathways are \textbf{not symmetric}.
As an analogy, let's consider the projection of a vector onto a direction. This can be formed as a dot product $\mathbf{v}\cdot \mathbf{n}$, where $\mathbf{v}$ stands for the vector to be projected and $\mathbf{n}$ is the unit vector representing the projection direction. The dot product is symmetric in its form. Nonetheless, $\mathbf{v}$ and $\mathbf{n}$ play distinct roles.
}\\

\q{The advantage of the two-pathway over the single-pathway models?}

\answer{The benefit of the two-pathway design comes from the explicit (and standalone) modeling of the geometric information. 
Despite single pathway models, such as TransGeo~\cite{transgeo} and L2LTR~\cite{l2ltr}, can explore the global spatial correlation among features, it is infeasible to tell how and to what extent such correlation is processed within those models.
On the opposite, the Geometric Layout Pathway in \ourmodel{} allows us to explicitly incorporate layout information, ensuring that the layout descriptors play a key role in constructing the final latent representation. Further, this enables us to utilize techniques like CF loss to enhance the quality of these descriptors.
It is worth noting that we do not rule out the possibility that a large model may handle the mixed representations and perform well in practice. Nonetheless, we believe that the information processing in GeoDTR+ will be much more efficient, enabling comparable performance with a much smaller parameter size as indicated in Table VII.
% \textcolor{red}{
% For example, TransGeo~\cite{transgeo}, SEH~\cite{SEH}, and L2LTR~\cite{l2ltr} rely on the single-pathway design to extract representations from the network. Single-pathway design can hardly disentangle the low-level features and spatial information, possibly resulting in overfitting to the training data (as shown in~\Cref{tab:corss_area}, most existing methods are under-performed). Besides that, to further strengthen the disentanglement, we apply the Counterfactual (CF) learning schema, and the Contrastive Hard Samples Generation (\chsg{}) techniques during training.}
}\\


\q{Ablation study to support the effectiveness of the proposed disentangled treatment}

\answer{Thanks for the suggestion. We agree that the activation function is a crucial part of our Geometric Layout Extractor to disentangle the information. However, simply removing the activation function only partially
% can hardly achieve the goal that 
``causing the information to be entangled again''
as the two-pathway design is left intact. 
% Since the geometric layout extractor is still learning to produce $\mathbf{q}'$ which can still partially disentangle the information. 
To support the above argument, we conduct two experiments. In the first experiment, as suggested, we remove the activation function of the geometric layout extractor and re-train the model. The results are presented in~\Cref{tab:activation_ablation}. We can observe that performance drops on both CVUSA and CVACT datasets, especially in cross-area experiments (i.e. R@1 decreases $3.82\%$ and $3.65\%$ on CVACT with and without polar transformation respectively). 

To further support our proposed two-pathway design, in the second experiment, we replace the $\mathbf{q}$ with all-ones descriptors during training. In this manner, all information in the raw features is contributed equally to the latent representation $f$. In this sense, \textbf{the Geometric Layout pathway is effectively muted}, breaking the disentanglement process. The results are illustrated in~\Cref{tab:all1_ablation}. We observe that replacing all-ones descriptors causes all performance to decrease drastically (i.e. R@1 decreases $8.62\%$ and $11.89\%$ on CVUSA with and without polar transformation respectively). These two experiments demonstrate the effectiveness of the proposed geometric layout extractor and our two-pathway design. For more experiment details, please refer to our Appendix(~\Cref{sec::ablation_GLD}).}\\

\q{(How) does the counterfactual (CF) learning schema contribute to the disentanglement?}

\answer{
The CF loss is incorporated to enhance the quality of geometric layout descriptors (GLDs) in the absence of ground truth descriptors. It punishes the artificially constructed fake descriptors and guides the training. In this sense, CF learning schema serves as a technique that complements our two-pathway design, requiring the existence of GLDs for enhancement. 
}\\

\q{Ablation study of CF.}

\answer{
Thanks for the suggestion. The CF learning schema was originally proposed in our preliminary work~\cite{GeoDTR} in which an ablation study was conducted to demonstrate its effectiveness. However, as suggested by the reviewer, we conduct an extra ablation study on the new \ourmodel{} to have a thorough study. The ablation study is presented in the Appendix(~\Cref{sec::ablation_CF}). \Cref{tab:CF_ablation} shows that the proposed CF improves both same-area and cross-area performance, especially on the cross-area evaluation protocol (i.e. on CVACT the R@1 decrease $4.16\%$ and $3.08\%$ while training with and without polar transformation respectively) which is aligned with our previous results~\cite{GeoDTR}. We also observe a stronger performance gain on the CVACT dataset than on the CVUSA dataset. We believe that this could be attributed to the saturation of the CVUSA dataset. For more experiment details, please refer to our Appendix(~\Cref{sec::ablation_CF}.)}\\


\q{Disentangling low-level features and spatial configuration via the transformer.}

\answer{Thanks for pointing this out. We realize that the original text implies that the disentanglement relies on the transformer. As we stated in the previous response, it is the two-pathway design rather than the transformer that enables the stand-alone treatment of the geometric layout. To address this confusion we modified the text as follows,}

\textbf{Before:} \textit{The above-mentioned methods implicitly model the spatial information from the raw features because solely rely on transformers. Nevertheless, \ourmodel{} not only explicitly models the local correlation but also explores the global contextual information through a transformer-based sub-module.}

\textbf{After:} \textit{
Despite the ability to explore spatial correlation, the above-mentioned methods do not process this global contextual information separately from others, such as the low-level features.
In this sense, they are of single-pathway nature.
Differently, our proposed \ourmodel{} employs a two-pathway design in which one pathway solely engages in the explicit modeling of global contextual information.
% Different from the above-mentioned methods which employ the single pathway design to implicitly model the local correlations, in this paper, our proposed \ourmodel{} employs a two-pathway design that disentangles the global contextual information from raw features. To achieve this, we propose a novel geometric layout extractor that explicitly models the global contextual information through a geometric layout extractor. The final latent representation is obtained through a modulation operation between the learned descriptors and raw features.
}\\

\q{Missing descriptions of the activation function of Geometric Layout Extractor in the Methodology section.}

\answer{Thanks for pointing this out. We have revised the paper as follows to include the description of the activation function we adopted to map the descriptors to the range $[0,1]$,}

\textbf{Before:} \textit{Finally, a bottleneck module consisting of two linear layers further refines $\mathbf{q'}$ and predicts GLDs $\mathbf{q}$.}

\textbf{After:} \textit{Finally, a bottleneck module consisting of two linear layers and an activation function refines $\mathbf{q'}$ and predicts GLDs $\mathbf{q}$. In the implementation, we choose the Sigmoid function as the activation function, which maps $\mathbf{q}' \in [-\infty,\infty]$ into $\mathbf{q} \in [0,1]$.}\\

==> text/response_old.tex <==
\textbf{\Large Summary of Changes} \\
% \begin{table*}[bp]
% 	\textcolor{red}{Author Response}
% \end{table*}

We would like to express our sincere gratitude to the reviewers for their insightful and constructive comments on our manuscript titled "GeoDTR\text{+}: Toward Generic Cross-View Geolocalization via Geometric Disentanglement" We appreciate the time and effort they dedicated to providing valuable suggestions for improving the quality and clarity of our paper.

We have revised the manuscript text, figures, and tables accordingly to enhance clarity and address any inconsistencies identified by the reviewers. We believe that these revisions have significantly strengthened the quality and impact of our work. In the remainder of this response, we provide a detailed account of the changes made and our responses to the reviewers' suggestions.

First of all, we would like to re-state the proposed architecture of the Geometric Layout Descriptor and relevant details of our \ourmodel{}. In \ourmodel{}, we argue that the stand-alone treatment of geometric layout would benefit the cross-view geo-localization task. This intuition is rooted in the fact that the relative spatial configuration of visual features remains invariant under view transformation, and there are geometric laws that constrain the mapping between different views. 
To explicitly utilize this spatial configuration, we propose the decomposition of the latent representation $f^v$ for view $v$ (for either aerial view or ground view),
$f^v$ = $q^v \circ r^v$ (\Cref{eq:main} in the manuscript),
where $q^v$ are the mask-like geometric layout descriptors, summarizing the spatial configuration of visual features, and $r^v$ denote raw latent representations from the backbone network. 
\textbf{We remark that,}
\begin{enumerate}
    \item $r^v$ includes information about both spatial configuration and low-level features (since it is extracted by backbone). However, these two types of information entangle with each other, preventing the model from efficiently exploiting the spatial configuration for matching images from different views.
    \item $q^v$ is mask-like and represents only the spatial configuration. In operation, a descriptor ‘selects’ (through modulation in~\Cref{eq:main}) specific areas from the raw latent representation for comparison. As a concrete example, let us consider an east-west road across the center of an aerial image. In the corresponding street-view image, this road will appear at the position of $\frac{1}{4}$ of width from the left side of the image and $\frac{3}{4}$ of width from the left side of the image. A descriptor could select features located in those areas and make the comparison between two views more efficient. Nonetheless, we also note that not all descriptors are meaningful to a human reader. Improving the interpretability of descriptors is a direction worth further investigation.
    \item Our model (\ourmodel{}) differs from conventional models in its two-pathway design that closely respects the proposed decomposition. The geometric layout pathway exclusively explores the spatial configuration of visual features. To do so, we employ standard transformer modules in this pathway to explore correlations among visual features more effectively, considering that the spatial configuration is a global property of visual features. On the other hand, existing transformer or CNN-based models follow a one-pathway design, and, without explicit processing, spatial configuration information is unavoidably mixed with low-level features. 
    \item In practice, there is no pre-defined ground-truth geometric layout descriptor. To address this issue in training, we introduce the counterfactual-based learning schema. Via penalizing the imaginary descriptors, the model can be away from apparently “wrong” solutions and learn better representation for descriptors.
    \item In this work, we explicitly model the geometric layouts as masks that select (through modulation) correlated visual features for comparison between different views. For individual views, corresponding descriptors have distinct representations, while, by design, capturing the same set of correlated visual features. In this way, we utilize the invariant spatial configuration information to facilitate efficient comparison.
\end{enumerate}

\noindent We realize that the original text may not adequately clarify the characteristics of our model and expect the above remarks to enhance comprehension of our work. Relevant descriptions will be updated in the revised version to reflect the above remarks.\\

\noindent\textbf{\textit{Responses to Reviewer 1:}}\\

\q{Why does using multi-head attention (of transformers) cause the undesired entanglement in TransGeo not in \ourmodel{}?}

\answer{In fact, the multi-head attention mechanism is not at the core of causing such an entanglement in TransGeo (or other single-pathway models). 
Instead, the model architecture is what matters.
In \ourmodel{}, it is the two-pathway design that disentangles the low-level features and the geometric layout descriptors rather than the adaptation of the transformer that enables the stand-alone treatment of the geometric layout. The geometric layout pathway generates representations regarding pure spatial configuration, thus, avoiding undesired entanglement with low-level features. 
For more details, please refer to remarks 1,2, and 3.}\\

\q{Does the raw feature $r^v$ already contain information about the spatial configuration? Can a CNN also model spatial configuration locally?}

\answer{1) Yes, the raw latent representations $r^v$ contain information about both the spatial configuration and low-level features. In GeoDTR+, we do not have a pathway that solely processes low-level features. 2) A CNN certainly can model spatial configuration. However, without explicitly separated processing, this information unavoidably entangles with others such as the low-level features. For more details, please refer to remarks 1, 2, and 3.}\\

\q{What causes the network to learn the ``spatial configuration'' in $q^v$ and "low-level features" in $r^v$?}

\answer{To enable the stand-alone treatment of spatial configuration, we incorporate a separate pathway for generating the geometric layout descriptors $q^v$ and the novel counterfactual learning schema (\Cref{sec::cf}) to supervise the training of these descriptors. As mentioned in~\Cref{sec::cf}, a good layout descriptor can be ``approximate'' by pushing the obviously wrong answer away in latent space. For more details, please refer to remark 4}\\

\q{What prevents the network from 1) representing spatial configuration in $r^v$ and low-level features in $q^v$ instead, or 2) mixing spatial configuration and low-level features in both $q^v$ and $r^v$.}

\answer{Descriptors $q^v$ do not represent low-level features since, first, they are mask-like feature maps whose elements take value in the range $[0,1]$; second, in our model design, these descriptors are used to select visual features from the raw latent representation and are not directly involved in comparing latent representations of different views. Hence, the model has no incentive to include information about low-level features in these descriptors.
3) The raw latent representations $r^v$ from the backbone networks mix spatial configuration and low-level features.
For more details, please refer to remarks 1,2, and 3.}\\

\q{Do the features learned in $r^v$ show a different distribution of activation? What kind of pattern of activation in an image would correspond with "low-level features".}

\answer{1) In \ourmodel{}, the raw latent representations $r^v \in \mathbb{R}^{C \times H \times W}$ ($C, H, W$ are channel, height, and width respectively) behave just like normal feature maps generated by a CNN network (as we adopt CNN-based backbone networks in the current work). $r^v$ contains information about \textbf{both the spatial configuration and low-level features}. For more details, please refer to remarks 1, 2, and 3.
2) The two-pathway design lies at the heart of the stand-alone extraction of the geometric layout. This design preserves in both GeoDTR and \ourmodel{}. In the current work, we modify the Geometric Layout Extractor (GLE) workflow to include more abundant local information from the backbone features, enabling the transformer module to better explore correlations among visual features at different locations. For more details, please refer to the last paragraph in~\Cref{sec::model}.
}\\

\q{What specifically makes an entanglement of low-level feature and spatial configuration undesirable anyway?}

\answer{We argue that the stand-alone modeling of spatial configuration would benefit the cross-view geo-localization task since this spatial configuration remains \textbf{invariant} under view transformation, thus helping efficient comparison between features. While previous (single pathway) methods (such as TransGeo~\cite{transgeo} and L2LTR~\cite{l2ltr}) capture as much information as ours, the spatial configuration therein mixes with low-level features, complicating the model's utilization of this valuable information. 
We do not rule out the possibility that a large model may handle the mixed representations and perform well in practice. Nonetheless, we believe that the information processing in GeoDTR+ will be much more efficient, enabling comparable performance with a much smaller parameter size as indicated in~\Cref{tab:computation}.
For more details, please refer to the overall response about GeoDTR+ and remarks 3 and 5.
}\\

\q{The architecture of the proposed \ourmodel{} does not seem to be an improvement over the preliminary GeoDTR.}

\answer{Thanks for pointing this out. We concur with the reviewer that the current ablation study does not clearly indicate the effectiveness of the new GLE. This may be because the performance in the same-area experiment is almost saturated on the CVUSA and the CVACT datasets, thus failing to accurately reflect the improvement of the novel GLE. Therefore, we conduct additional experiments on the VIGOR dataset (\Cref{tab:VIGOR_ablation}) for a more comprehensive demonstration of the contribution of GLE in our model. Specifically, our GLE improves from $55.14\%$ to $59.01\%$ on R@1 in the same-area experiment with ConvNext backbone and training with CHSG. While without CHSG, our GLE improves from $56.63\%$ to $58.46\%$ on R@1. We also observed that without CHSG, the new GLE might slightly decrease the cross-area performance. Thus, we suggest applying both the new GLE and CHSG at the same time when training the model. In summary, from our ablation study on VIGOR, we can see that the proposed novel GLE improves the same-area performance constantly. While training with \chsg{}, it can improve both same-area and cross-area performance.}\\

\q{It is unclear whether the proposed model architecture represents an improvement over architectures from related works (e.g. SAIG).}

\answer{Thanks for pointing this out. We carry out new experiments on CVUSA and CVACT datasets to investigate whether the model architecture of GeoDTR+ presents an improvement over SAIG. First, we updated~\Cref{tab:same_area}, \Cref{tab:corss_area}, and~\Cref{tab:vigor} with SAIG model. As we can see, our \ourmodel{} outperforms SAIG in both same-area and cross-area experiments on CVUSA and CVACT benchmarks. Especially on the cross-area experiment, our \ourmodel{} outperforms SAIG by $44.87\%$ on R@1 of CVUSA $\rightarrow$ CVACT and $33.59\%$ on R@1 of CVACT $\rightarrow$ CVUSA. Moreover, we compared the two methods at the raw network level (i.e., both without CHSG) as well as the full model level (i.e., both with CHSG) in~\Cref{tab:archietecture_comparison}. As demonstrated in the experiment, 1) On both CVUSA and CVACT datasets, it is worth noting that GeoDTR+ beats SAIG on both same-area ($94.09\%$ vs $92.71\%$ on CVUSA same-area without \chsg{}) and cross-area ($60.16\%$ vs $26.82\%$ on CVUSA $\rightarrow$ CVACT without \chsg{}) performance regardless of whether applying CHSG (with only one exception on CVACT same-are experiment). 2) The results indicate that our CHSG can notably enhance cross-area accuracy across various methods while having only a minor impact on same-area performance.}\\

\q{SAFA also uses a global aggregation scheme and can explore spatial layout.}

\answer{Thanks for pointing out this ambiguous claim. We agree that SAFA can explore spatial configurations. We mention the limit of SAFA because it explores the spatial configuration using fully connected layers, which normally can hardly and implicitly capture global correlations among visual features compared to the Transformer that is employed in our \ourmodel{}. The fully connected layer is often considered less effective at capturing input data correlations compared to transformer layers. We modified the text as follows,

\textbf{Before: }\textit{For example, Spatial-Aware Feature Aggregation (SAFA)~\cite{SAFA} proposed to explore the CNN extracted feature by a customized Spatial-aware Positional Embedding (SPE) module. Such methods are limited in exploring the spatial configuration which is a global property (i.e. a highway spanning west to east on an aerial image) due to the tendency to explore local correlations among pixels in CNNs. }

\textbf{After: }\textit{For example, Spatial-Aware Feature Aggregation (SAFA)~\cite{SAFA} proposed to explore the CNN extracted feature by a customized Spatial-aware Positional Embedding (SPE) module which explores the spatial configuration by fully connected layers. Such methods are limited in exploring the spatial configuration which is a global property (i.e. a highway spanning west to east on an aerial image) due to the capacity of fully connected layers that can hardly explore correlations explicitly.}} \\

\q{Why do more concentrated regions imply a more distinguishable latent representation?}

\answer{The latent representations are obtained through the modulation operation between geometric layout descriptors and the raw latent representation (see~\Cref{eq:main}). Thus, in the training stage, the raw latent representation and geometric layout descriptors are optimized concurrently to match each other. Moreover, more concentrated layout descriptors imply that one needs fewer dimensions in the learned raw latent representations to distinguish the two views. Finally, \ourmodel{} outperforms our preliminary GeoDTR. Combining all the above three points, we see that \ourmodel{} learns raw latent representations that enable better performance with less dimension used for matching. In this sense, we claim the \ourmodel{} learns a more distinguishable latent representation. We modified the corresponding text as follows, 

\textbf{Before: }\textit{It is clear to see that despite the polar transformation, \ourmodel{} learns more concentrated regions than GeoDTR which implies that \ourmodel{} learns a more distinguishable latent representation.}

\textbf{After: }\textit{It is clear to see that despite the polar transformation, \ourmodel{} learns more concentrated regions than GeoDTR which implies that fewer dimensions in the learned raw latent representations are needed to distinguish the aerial and ground views. By combining the overall performance improvement from GeoDTR to \ourmodel{}, it implies that \ourmodel{} learns a more distinguishable latent representation.}}\\

\q{Why the observation that our \ourmodel{} training without polar transformation outperforms other models with polar transformation can be attributed to the proposed GLE?}

\answer{Thanks for pointing this out. The cited claim (P7 L24) was made under the situation “Without polar transformation” (P7 L18). In that paragraph, we emphasize that the results of GeoDTR+ without polar transformation outperform others with polar transformation (and are close to the performance of GeoDTR+ with polar transformation). This is not observed in our previous work, i.e., GeoDTR, and thus cannot be attributed to LS. We modify the corresponding text as follows, 

\textbf{Before: }\textit{Notably, on CVACT\_val and CVACT\_test, the proposed model not only achieves SOTA performance but also outperforms results trained with polar transformation, which is not observable in other methods such as SAFA~\cite{SAFA} and L2LTR~\cite{l2ltr}. This can be attributed to the ability of the proposed novel Geometric Layout Extractor (GLE) to explore global spatial configurations.}

\textbf{After: }\textit{Notably, on CVACT\_val and CVACT\_test, our \ourmodel{} without polar transformation not only achieves SOTA performance but also outperforms other models trained with polar transformation, which is not observable in other methods such as SAFA~\cite{SAFA} and L2LTR~\cite{l2ltr}. We attribute this to the ability of the proposed novel Geometric Layout Extractor (GLE) to explore global spatial configurations.}}\\

\q{What is the reasoning for ``the current emphasis within the CVGL field is primarily placed on improving same-area performance [5], [6], [14].''?}

\answer{Thanks for pointing out this ambiguity. We agree that more recent methods are evaluated on cross-area benchmarks. However, these methods cannot achieve satisfactory performance in cross-area benchmarks. On the other hand, our proposed \ourmodel{} is more focused on improving the cross-area evaluation which is a more challenging setting. And our results in~\Cref{tab:corss_area,tab:vigor} demonstrate the superiority of our model on cross-area evaluation. We modified the text as follows, 

\textbf{Before: }\textit{the current emphasis within the CVGL field is primarily placed on improving same-area performance~\cite{SAFA,cvmnet,DSM}.}

\textbf{After: }\textit{the current emphasis within the CVGL field is primarily placed on improving same-area performance~\cite{SAFA,cvmnet,DSM,transgeo,SAIG}. However, there is a lack of a method for generalizing the model on cross-area benchmarks.}
}\\

\q{Why does not tuning the full backbone feature make training easier?}

\answer{Thanks for pointing out this vague expression. In \ourmodel{}, the geometric layout descriptors select those areas in the latent representation that are discriminative for comparing two views. Only those areas receive significant gradient signals during back-propagation, making the model training more targeted. In this way, the model potentially learns better latent representation. We modified the corresponding text as follows,

\textbf{Before: }\textit{Second, only elements within the active areas receive significant gradients signal during back-propagation. This makes the training easier as it needs not to tune the full backbone feature.}

\textbf{After: }\textit{Second, only elements within the active areas receive significant gradient signals during back-propagation. This makes the model training more targeted to focus on discriminative features, resulting in the model easier to learn better latent representations.}}\\

\q{Figure captions in~\Cref{fig:latent_feature_difference} and~\Cref{tab:GLE} are hard to understand.}

\answer{We change the capture of~\Cref{fig:latent_feature_difference} to ``Visualization of the distributions of latent feature distances using violin plot of our \ourmodel{} training with \chsg{} and training without \chsg{} on $200$ random test aerial-ground pairs.'' for better readability. For~\Cref{fig:latent_feature_difference}, and other tables with both training on CVUSA and CVACT datasets, we added ``Training Set'' to the top of the column to inform the audience of the training and testing part for each experiment.}\\

\q{Problem formulation in one-to-one matching.}

\answer{Thanks for pointing this out. We updated the relevant text (in the introduction and methodology sections) to incorporate one-to-many matching in cross-view geo-localization.}\\

\q{The difference between feature-based and geometry-based cross-view geo-localization methods in related work section.}

\answer{Thanks for pointing this out. We added the following text to define these two categories in~\Cref{sec::related_works_CVGL},}

\textit{1) Feature-based geo-localization methods extract both aerial and ground latent representations from local information using hand-crafted features or deep learning models without any geometric priors~\cite{lin2013cross, lin2015learning, CVUSA, survey}.}

\textit{2) Recently, learning to match the geometric correspondence between aerial and street views has become a hot topic in cross-view geo-localization. Specifically, these methods leverage geometric priors such as polar transformation, heading, and orientation information or learning to capture non-local correlations to better predict the similarities in aerial and ground latent featuers~\cite{survey}.}\\

\q{Typos and languages can be improved.}

\answer{Thanks for pointing out these errors. We have updated the text accordingly.}\\

\noindent\textbf{\textit{Responses to Reviewer 2:}}\\

\q{Missing citations of two recently proposed papers in the related work section.}

\answer{Thanks for pointing out these two recent papers. We have added the following text in~\Cref{sec::related_works_CVGL} to discuss these two relevant papers,}

\textit{TGCNN~\cite{TGCNN} adopted transformers to explore global and local correlations simultaneously. MGTL~\cite{MGTL} leveraged mutual interaction between aerial and ground images from a customized transformer mudle.}\\

\q{Missing comparison results of two recently proposed papers in main results table.}

\answer{Thanks for pointing this out. We have updated the~\Cref{tab:same_area} in the manuscript by including TGCNN and MGTL.}\\

\q{More experiments and analysis on VIGOR dataset.}

\answer{Thanks for your suggestion. We conducted additional ablation studies of our \ourmodel{} on VIGOR datasets with same-area and cross-area evaluation protocols. The results are presented in the newly added appendix section in~\Cref{tab:VIGOR_ablation}. By comparing different GLEs with the same backbone and CHSG configurations in~\Cref{tab:VIGOR_ablation}, we can see that the new GLE improves the same-area performance, for example with ResNet-34 backbone and without \chsg{}, R@1 increases from $56.51\%$ to $57.24\%$ and $55.14\%$ to $59.01\%$ with ConvNext-Tiny backbone and training with \chsg{}. We also observed that \chsg{} significantly boosts the cross-area performance, especially on the ConvNext-Tiny backbone (i.e. R@1 increases from $26.15\%$ to $36.01\%$). However, it is noted that the proposed new GLE can improve same-area performance while slightly decreasing cross-area performance when training without \chsg{} (i.e. while training with ConvNext-Tiny and without \chsg{}, the R@1 decreases from $27.04\%$ to $26.15\%$). This slight decrease can be attributed to the new GLE that better captures the spatial correlations in the input images which might cause the model overfitting to them. Thus, we suggest applying both the new GLE and CHSG at the same time when training the model to obtain the best performance.}\\

\noindent\textbf{\textit{Response for common reviews from both R1 and R2:}}\\

\q{The statements of the performance on the VIGOR dataset.}
\answer{Thanks for pointing this out. We agree that there is a gap between our \ourmodel{} and the SOTA method the same-area benchmark of VIGOR. However, we want to point out that we trade off this slight same-area performance drop to a significant cross-area performance increase. Also, in~\Cref{tab:chsg_LS_batch} and~\Cref{tab:chsg}, there is only a slight decrease in same-area performance (less than $1\%$ on R@1) but a significant improvement in cross-area performance (around $8\%$) when applying our proposed \chsg{}. Thus, our statement, ``Results in Tables~\Cref{tab:chsg_LS_batch} and~\Cref{tab:chsg}I confirm the benefits of CHSG on our model, especially the improvement in cros-sarea performance.'', still holds. Most importantly, in~\Cref{sec::computational_efficiency}, we illustrate that \ourmodel{} is the smallest model among all the baselines. In other words, the same-area performance can further improve if a larger backbone is employed (for example applying ConvNext-Base~\cite{convnext} which has 4 times more parameters than the employed ConvNext-Tiny~\cite{convnext} backbone in this paper). However, this is not the focus of this paper.  We added the following text in~\Cref{sec::main_results} 3) to further explain these points,}

\textit{The same-area performance difference might come from both model scale and the augmentation in \chsg{} such as the color space distortion and geometric transformations. In summary, \ourmodel{} shows significantly enhances the cross-area performance over the SOTA methods on cross-area evaluation. Although, there is a slight drop in same-area evaluation. However, in later~\Cref{sec::computational_efficiency}, we show that \ourmodel{} is the smallest model among all the baseline methods. Thus 
the same-area performance can be further improved by applying a larger backbone. However, it is not the focus of this paper.}

And updated the following text to explain the results more precisely,

\textbf{Before: } \textit{As we can see that training with the novel GLE (v2) on ResNet-34 [40] improves the cross-area performance on both CVUSA and CVACT datasets}

\textbf{After: }\textit{ As we can see training with the novel GLE (v2) on ResNet-34~\cite{resnet} generally improves the cross-area performance on both CVUSA and CVACT datasets (except while training with \chsg{} on the CVACT, there is a slight drop from $50.63\%$ to $49.09\%$). For example, the \Rone{} accuracy improves from $57.03\%$ (line 1) to $59.72\%$ (line 3) on the CVUSA dataset.} 
